Uncertainty with UAV Search of Multiple Goal-oriented Targets

This paper considers the complex problem of a team of UAVs searching targets under uncertainty. The goal of the UAV team is to find all of the moving targets as quickly as possible before they arrive at their selected goal. The uncertainty considered is threefold: First, the UAVs do not know the targets' locations and destinations. Second, the sensing capabilities of the UAVs are not perfect. Third, the targets' movement model is unknown. We suggest a real-time algorithmic framework for the UAVs, combining entropy and stochastic-temporal belief, that aims at optimizing the probability of a quick and successful detection of all of the targets. We have empirically evaluated the algorithmic framework, and have shown its efficiency and significant performance improvement compared to other solutions. Furthermore, we have evaluated our framework using Peer Designed Agents (PDAs), which are computer agents that simulate targets and show that our algorithmic framework outperforms other solutions in this scenario.

==> question_letter.tex <==

\begin{enumerate}
    \item What is the main claim of the paper? Why is this an important contribution to the autonomous agents and multi-agent systems literature?
    
    In this paper, we introduce a new problem that considers the uncertainty with UAV search Of MultiplE Goal-oriented tArgets (OMEGA). In OMEGA, the UAVs' goal is to search and detect the targets, where the sensing capabilities of the UAVs are imperfect. The mobile targets are grounded, and their objective is to reach one of the goals. In OMEGA, multiple targets can enter from various locations. Each target can have a different movement model. A target chooses its goal at random, and this chosen goal is unknown to the UAVs. The target travels in the environment according to a (probabilistic) noisy movement model.
    
    \item What is the evidence you provide to support your claim? 
    In this paper: we provide efficient algorithms for solving realistic OMEGA and MTS problems which include:
    1) A general graph, not a grid, which can cope with environmental constraints such as a no flying zone.
    2) Goal-oriented targets.
    3) Heterogeneous targets and UAVs.
    4) Multiple targets with different initial locations.
    5) Diverse movement strategies (known and unknown strategies). 
    6) UAVs with imperfect detection capabilities.
    7) Moving targets, not static ones.
    
    \item Have you published parts of your paper before, for instance in a conference? If so, give details of your previous paper(s) and a precise statement detailing how your paper provides a significant contribution beyond the previous paper(s).
    
    Initial results of a less complicated problem were presented in previous work \cite{sinay2018uav}. In this paper, the UAVs and the targets are heterogeneous with respect to their movement capabilities. Furthermore, we use diverse targets, with different movement models that enter from various different locations. We use a distinct probabilistic belief model for each target.
    We built a realistic border defense simulation demonstrating its high success rate in the detection of the targets, empirically evaluated our algorithm with extensive simulations and present its efficiency for targets with a {\em known} strategy and an {\em unknown} strategy using Peer Designed Agents (PDAs).
    
\end{enumerate}


